Spacetime Representation Theory: Setting the Scope of the ISE Method of Topological Redescription

Spacetime dualities arise whenever two theories -- despite being structurally equivalent in some sense -- seemingly provide us with two radically different spatiotemporal descriptions of the world. This often involves radical differences in how the two theories topologically stage their states; Whereas one theory is about *this* type of particle/field on *this* smooth manifold, the other theory is about *that* type of particle/field arranged differently on *that* smooth manifold. For instance, the AdS-CFT correspondence relates a certain theory set in the bulk (our 3+1 dimensional spacetime) to another theory set on the boundary (a 2+1 dimensional spacetime). Another example (new in this paper) is the M\"{o}bius-Euclid duality: a theory about a certain type of particle floating around on the Euclidean plane can be topologically redescribed as instead being about a different type of particle living on a M\"{o}bius strip, and vice versa. The possibility of such alternative spacetime framings raises some significant questions about the epistemology and metaphysics of space and time. For instance, what are our topology selection criteria? Are they objective or conventional? Moreover, given that two spacetime theories are topological redescriptions of each other, what is the common core which they are equivalent descriptions of? As a step towards answering such questions, this paper develops a general framework (spacetime representation theory) for understanding our ability to topologically redescribe our spacetime theories. With this framework established, I will then discuss the ISE Equivalence Theorem which sets the scope of the recently developed ISE Method of topological redescription.

==> references.tex <==
@misc{Pooley2015,
	Archiveprefix = {arXiv},
	Author = {Pooley, Oliver},
	Eprint = {1506.03512},
	Primaryclass = {gr-qc},
	Slaccitation = {%%CITATION = ARXIV:1412.7827;%%},
	Title = {{Background Independence, Diffeomorphism Invariance, and the Meaning of Coordinates}},
	Year = {2015},
	url = {https://arxiv.org/abs/1506.03512}}

@article{EinsteinFokker,
issn = {0003-3804},
journal = {Annalen der Physik},
language = {ger},
number = {10},
author = {Einstein, A. and Fokker, A. D.},
address = {Leipzig},
title = {{Die Nordströmsche Gravitationstheorie vom Standpunkt des absoluten Differentialkalküls}},
volume = {349},
year = {1914},
pages = {321-328},
publisher = {WILEY-VCH Verlag},
}

@article{Norton1993,
	doi = {10.1088/0034-4885/56/7/001},
	year = 1993,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {56},
	number = {7},
	pages = {791--858},
	author = {John D. Norton},
        title = {General covariance and the foundations of general relativity: eight decades of dispute},
	journal = {Reports on Progress in Physics},
	abstract = {Einstein offered the principle of general covariance as the fundamental physical principle of his general theory of relativity and as responsible for extending the principle of relativity to accelerated motion. This view was disputed almost immediately with the counter-claim that the principle was no relativity principle and was physically vacuous. The disagreement persists today. This article reviews the development of Einstein's thought on general covariance, its relation to the foundations of general relativity and the evolution of the continuing debate over his viewpoint.}
}

@article{SaundersSimon2013RNP,
language = {eng},
number = {1},
pages = {22-48},
publisher = {University of Chicago Press},
title = {{Rethinking Newton's Principia}},
volume = {80},
year = {2013},
author = {Saunders, Simon},
address = {Chicago, IL},
copyright = {Copyright 2013 by the Philosophy of Science Association. All rights reserved.},
issn = {0031-8248},
journal = {Philosophy of Science},
keywords = {Mechanics ; Philosophy ; Physics ; Sociology ; Space ; Time},
}

@incollection{Friedman1983,
    author = {Michael Friedman},
    editor = {ibid.},
    booktitle = {Foundations of Space-Time Theories: Relativistic Physics and Philosophy of Science},
    publisher = {Princeton University Press},
    title = {{Space-Time Theories}},
    year = {1983},
    chapter = {2},
    pages = {32-70},
}
 
@article{Teitel2019,
issn = {1355-2198},
journal = {Studies In History And Philosophy Of Modern Physics},
pages = {pp41--54},
volume = {65},
publisher = {Elsevier Ltd},
year = {2019},
title = {Background independence: Lessons for further decades of dispute},
copyright = {legaldeposit},
author = {Teitel, Trevor},
keywords = {530.01; Physics--History--Periodicals; Physics--Philosophy--Periodicals},
}

@inbook{Pooley2010,
 URL = {http://www.jstor.org/stable/j.ctt7ztj02.5},
 author = {Oliver Pooley},
 booktitle = {EPSA philosophical issues in the sciences},
 pages = {197--210},
 chapter = {19}, 
 publisher = {Springer},
 title = {Space-Time Theories},
 isbn = {9789048132515},
 year = {2010},
 address = {Dordrecht ; London},
 editor = {Suárez, Mauricio and Dorato, Mauro and Rédei, Miklós}
}

@mastersthesis{ReadThesis,
  year = {2016},
  edition = {},
  number = {},
  journal = {},
  pages = {},
  publisher = {University of Oxford},
  school = {University of Oxford},
  title = {Background independence in classical and quantum gravity},
  volume = {},
  author = {Read, James},
  editor = {},
  series = {}
}

@article{Pitts2006,
issn = {1355-2198},
journal = {Studies in History and Philosophy of Modern Physics},
pages = {347--371},
volume = {37},
publisher = {Elsevier Ltd},
number = {2},
year = {2006},
title = {Absolute objects and counterexamples: Jones–Geroch dust, Torretti constant curvature, tetrad-spinor, and scalar density},
author = {Brian Pitts, J},
keywords = {Absolute Object ; General Covariance ; Spinor ; Tetrad ; Unimodular ; Density ; Absolute Object ; General Covariance ; Spinor ; Tetrad ; Unimodular ; Density ; Sciences (General) ; Philosophy ; Physics},
}

@article{Belot2011,
issn = {0001-7701},
journal = {General Relativity and Gravitation},
pages = {2865--2884},
volume = {43},
publisher = {Springer US},
number = {10},
year = {2011},
title = {Background-independence},
address = {Boston},
author = {Belot, Gordon},
keywords = {Background-independence ; General relativity ; Absolute objects},
}

@book{EarmanJohn1989Weas,
publisher = {MIT Press},
isbn = {9780262050401},
year = {1989},
title = {{World Enough and Space-Time: {A}bsolute versus Relational Theories of Space and Time}},
author = {Earman, John},
keywords = {Absolute, The; Relationism; Science -- Methodology -- Philosophy; Science -- Philosophy; Space and time},
lccn = {LC},
}

@misc{TehFreidel,
    title={Substantive general covariance and the Einstein-Klein dispute: A Noetherian approach},
    author={Freidel, Laurent and Tah, Nicholas},
    year={2021},
    eprint={2109.08516},
    archivePrefix={arXiv},
    primaryClass={hist-ph},
    url={https://arxiv.org/abs/2109.08516}
}

@article{WallaceAfraid,
	publisher = {Elsevier Bv},
	volume = {67},
	author = {David Wallace},
	title = {Who's Afraid of Coordinate Systems? An Essay on Representation of Spacetime Structure},
	journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
	year = {2019},
	doi = {10.1016/j.shpsb.2017.07.002},
	pages = {125--136}
}

@article{ThorneLeeLightman,
  title = {Foundations for a Theory of Gravitation Theories},
  author = {Thorne, Kip S. and Lee, David L. and Lightman, Alan P.},
  journal = {Phys. Rev. D},
  volume = {7},
  issue = {12},
  pages = {3563--3578},
  numpages = {0},
  year = {1973},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.7.3563},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.7.3563}
}

@article{Janotta_2014,
	doi = {10.1088/1751-8113/47/32/323001},
	url = {https://doi.org/10.1088/1751-8113/47/32/323001},
	year = 2014,
	month = {jul},
	publisher = {{IOP} Publishing},
	volume = {47},
	number = {32},
	pages = {323001},
	author = {Peter Janotta and Haye Hinrichsen},
	title = {Generalized probability theories: what determines the structure of quantum theory?},
	journal = {Journal of Physics A: Mathematical and Theoretical},
	abstract = {The framework of generalized probabilistic theories is a powerful tool for studying the foundations of quantum physics. It provides the basis for a variety of recent findings that significantly improve our understanding of the rich physical structure of quantum theory. This review paper tries to present the framework and recent results to a broader readership in an accessible manner. To achieve this, we follow a constructive approach. Starting from a few basic physically motivated assumptions we show how a given set of observations can be manifested in an operational theory. Furthermore, we characterize consistency conditions limiting the range of possible extensions. In this framework classical and quantum theory appear as special cases, and the aim is to understand what distinguishes quantum mechanics as the fundamental theory realized in nature. It turns out that non-classical features of single systems can equivalently result from higher-dimensional classical theories that have been restricted. Entanglement and non-locality, however, are shown to be genuine non-classical features.}
}

@article{pub.1136830387,
 abstract = {SciPost Journals Publication Detail SciPost Phys. Lect. Notes 28 (2021) Probabilistic theories and reconstructions of quantum theory},
 author = {Müller, Markus},
 doi = {10.21468/scipostphyslectnotes.28},
 journal = {SciPost Physics Lecture Notes},
 keywords = {},
 note = {https://scipost.org/10.21468/SciPostPhysLectNotes.28/pdf},
 number = {},
 pages = {028},
 title = {Probabilistic theories and reconstructions of quantum theory},
 url = {https://app.dimensions.ai/details/publication/pub.1136830387},
 volume = {},
 year = {2021}
}

@article{pub.1143048427,
 abstract = {Gleason-type theorems for quantum theory allow one to recover the quantum state space by assuming that (i) states consistently assign probabilities to measurement outcomes and that (ii) there is a unique state for every such assignment. We identify the class of general probabilistic theories which also admit Gleason-type theorems. It contains theories satisfying the no-restriction hypothesis as well as others which can simulate such an unrestricted theory arbitrarily well when allowing for post-selection on measurement outcomes. Our result also implies that the standard no-restriction hypothesis applied to effects is not equivalent to the dual no-restriction hypothesis applied to states which is found to be less restrictive.},
 author = {Wright, Victoria J and Weigert, Stefan},
 doi = {10.22331/q-2021-11-25-588},
 journal = {Quantum},
 keywords = {},
 note = {https://quantum-journal.org/papers/q-2021-11-25-588/pdf/},
 number = {},
 pages = {588},
 title = {General Probabilistic Theories with a Gleason-type Theorem},
 url = {https://app.dimensions.ai/details/publication/pub.1143048427},
 volume = {5},
 year = {2021}
}

@article{pub.1135756008,
 abstract = {},
 author = {Shahandeh, Farid},
 doi = {10.1103/prxquantum.2.010330},
 journal = {PRX Quantum},
 keywords = {},
 note = {http://link.aps.org/pdf/10.1103/PRXQuantum.2.010330},
 number = {1},
 pages = {},
 title = {Contextuality of General Probabilistic Theories},
 url = {https://app.dimensions.ai/details/publication/pub.1135756008},
 volume = {2},
 year = {2021}
}

@article{pub.1105420091,
 abstract = {Jeff Bub has developed an information-theoretic interpretation of quantum mechanics on the basis of the programme to reaxiomatise the theory in terms of information-theoretic principles. According to the most recent version of the interpretation, reaxiomatisation can dissolve some of the demands for explanation traditionally associated with the task of providing an interpretation for the theory. The key idea is that the real lesson we should take away from quantum mechanics is that the ‘structure of information’ is not what we thought it was. In particular a feature of the new structure is intrinsic randomness of measurement, which allegedly dissolves a significant part of the measurement problem. I argue that it is difficult to find an appropriate argument to support the claim that measurement is intrinsically random in the relevant sense.},
 author = {Henderson, Leah},
 doi = {10.1016/j.shpsb.2018.06.003},
 journal = {Studies in History and Philosophy of Science Part A},
 keywords = {},
 number = {},
 pages = {292-300},
 title = {Quantum reaxiomatisations and information-theoretic interpretations of quantum theory},
 url = {https://app.dimensions.ai/details/publication/pub.1105420091},
 volume = {72},
 year = {2020}
}

@article{pub.1052891771,
 abstract = {The aim of this paper is to consider the consequences of an information-theoretic interpretation of quantum mechanics for the measurement problem. The motivating idea of the interpretation is that the relation between quantum mechanics and the structure of information is analogous to the relation between special relativity and the structure of space-time. Insofar as quantum mechanics deals with a class of probabilistic correlations that includes correlations structurally different from classical correlations, the theory is about the structure of information: the possibilities for representing, manipulating, and communicating information in a genuinely indeterministic quantum world in which measurement outcomes are intrinsically random are different than we thought. Part of the measurement problem is deflated as a pseudo-problem on this view, and the theory has the resources to deal with the remaining part, given certain idealizations in the treatment of macrosystems.},
 author = {Bub, Jeffrey},
 doi = {10.3390/e17117374},
 journal = {Entropy},
 keywords = {},
 note = {https://www.mdpi.com/1099-4300/17/11/7374/pdf},
 number = {11},
 pages = {7374-7386},
 title = {The Measurement Problem from the Perspective of an Information-Theoretic Interpretation of Quantum Mechanics},
 url = {https://app.dimensions.ai/details/publication/pub.1052891771},
 volume = {17},
 year = {2015}
}

@inbook{pub.1104045230,
 abstract = {},
 author = {Koberinski, Adam and Müller, Markus P.},
 booktitle = {Physical Perspectives on Computation, Computational Perspectives on Physics},
 doi = {10.1017/9781316759745.013},
 keywords = {},
 note = {http://arxiv.org/pdf/1707.05602},
 pages = {257-280},
 publisher = {Cambridge University Press},
 title = {Quantum Theory as a Principle Theory: Insights from an Information-Theoretic Reconstruction},
 url = {https://app.dimensions.ai/details/publication/pub.1104045230},
 year = {2018}
}

@inbook{rovelli_2001, place={Cambridge}, title={Quantum spacetime: What do we know?}, DOI={10.1017/CBO9780511612909.005}, booktitle={Physics Meets Philosophy at the Planck Scale: Contemporary Theories in Quantum Gravity}, publisher={Cambridge University Press}, author={Rovelli, Carlo}, editor={Callender, Craig and Huggett, Nick}, year={2001}, pages={101–122}}

@book{rovelli_2004, place={Cambridge}, series={Cambridge Monographs on Mathematical Physics}, title={Quantum Gravity}, DOI={10.1017/CBO9780511755804}, publisher={Cambridge University Press}, author={Rovelli, Carlo}, year={2004}, collection={Cambridge Monographs on Mathematical Physics}}

@incollection{SmolinLee2006TCfB,
abstract = {This chapter explains the arguments behind the assertion that the correct quantum theory of gravity must be background independent. It begins by recounting how the debate over whether quantum gravity must be background independent is a continuation of a long-standing argument in the history of physics and philosophy over whether space and time are relational or absolute. This leads to a careful statement of what physicists mean when we speak of background independence. Given this we can characterize the precise sense in which general relativity is a background-independent theory. The leading background-independent approaches to quantum gravity are then discussed, including causal set models, loop quantum gravity, and dynamical triangulations, and their main achievements are summarized along with the problems that remain open. The relational/absolute debate has implications also for other issues such as unification and how the parameters of the standard models of physics and cosmology are to be explained. The chapter reviews recent issues concerning the string theory landscape and argues that they can only be resolved within the context of a background-independent formulation. Finally, it reviews some recent proposals to make quantum theory more relational.},
publisher = {Oxford University Press},
booktitle = {The Structural Foundations of Quantum Gravity},
isbn = {0199269696},
year = {2006},
title = {The Case for Background Independence},
copyright = {Copyright 2015 Elsevier B.V., All rights reserved.},
address = {Oxford},
author = {Smolin, Lee},
keywords = {Background independence ; Quantum theory ; Reductionism ; Relationalism ; Space ; String theory ; Time},
}

@book{SmolinLee2008Ttwp,
publisher = {Penguin},
isbn = {9780141018355},
year = {2008},
title = {The trouble with physics: the rise of string theory, the fall of a science and what comes next},
address = {London},
author = {Smolin, Lee},
keywords = {String models -- Popular works; Physics -- Methodology -- History},
}

@article{deHaroSebastian2017Daeg,
issn = {1355-2198},
journal = {Studies in History and Philosophy of Modern Physics},
pages = {109--125},
volume = {59},
publisher = {Elsevier Ltd},
year = {2017},
title = {Dualities and emergent gravity: Gauge/gravity duality},
copyright = {2015 Elsevier Ltd},
address = {OXFORD},
author = {de Haro, Sebastian},
keywords = {Analysis ; Arts & Humanities ; Duality ; Emergence ; Gauge/gravity duality ; Gravity ; History & Philosophy Of Science ; Holography ; Physical Sciences ; Physics ; Physics, Multidisciplinary ; Quantum gravity ; Science & Technology ; String theory},
}

@article{DeHaroSebastian2017TIoD,
issn = {0015-9018},
journal = {Foundations of physics},
pages = {1464--1497},
volume = {47},
publisher = {Springer US},
number = {11},
year = {2017},
title = {The Invisibility of Diffeomorphisms},
copyright = {The Author(s) 2017},
address = {New York},
author = {De Haro, Sebastian},
keywords = {Ambient construction ; Article ; Asymptotic symmetries ; Classical and Quantum Gravitation ; Classical and Quantum Gravitation, Relativity Theory ; Classical Mechanics ; Conformal geometry ; Diffeomorphism invariance ; Gauge–gravity duality ; Gravitation ; Gravity ; History and Philosophical Foundations of Physics ; Philosophy of Science ; Philosophy of string theory ; Physical Sciences ; Physics ; Physics and Astronomy ; Physics, Multidisciplinary ; Quantum gravity ; Quantum Physics ; Relativity ; Relativity Theory ; Science & Technology ; Statistical Physics and Dynamical Systems ; Visibility},
}

@misc{CurvedSampling,
    title={Geometric Space-Frequency Analysis on Manifolds},
    author={Feichtinger, Hans G. and Führ, Hartmut and Pesenson, Isaac Z.},
    year={2015},
    eprint={1512.08668},
    archivePrefix={arXiv},
    primaryClass={math.FA},
    url={https://arxiv.org/abs/1512.08668}
}

@Article{Martin2008,
author={Martin, R.
and Kempf, A.},
title={Approximation of Bandlimited Functions on a Non-Compact Manifold by Bandlimited Functions on Compact Submanifolds},
journal={Sampling Theory in Signal and Image Processing},
year={2008},
month={Sep},
day={01},
volume={7},
number={3},
pages={281-292},
issn={1530-6429},
doi={10.1007/BF03549501},
url={https://doi.org/10.1007/BF03549501}
}

@incollection{GARCIA200263,
title = {A Brief Walk Through Sampling Theory},
editor = {Peter W. Hawkes},
series = {Advances in Imaging and Electron Physics},
booktitle = {Advances in Imaging and Electron Physics Vol 124},
publisher = {Elsevier},
volume = {124},
pages = {63-137},
year = {2002},
issn = {1076-5670},
doi = {https://doi.org/10.1016/S1076-5670(02)80042-8},
url = {https://www.sciencedirect.com/science/article/pii/S1076567002800428},
author = {Antonio G. García}
}

@INPROCEEDINGS{ReconstructionStability,
  author={Hao, Yufang and Kempf, Achim},
  booktitle={2008 International Symposium on Information Theory and Its Applications}, 
  title={On the stability of a generalized Shannon sampling theorem}, 
  year={2008},
  volume={},
  number={},
  pages={1-6},
  doi={10.1109/ISITA.2008.4895514}}
  
@ARTICLE{SamplingTutorial,  author={Jerri, A.J.},  journal={Proceedings of the IEEE},   title={The Shannon sampling theorem—Its various extensions and applications: A tutorial review},   year={1977},  volume={65},  number={11},  pages={1565-1596},  doi={10.1109/PROC.1977.10771}}

@article{UnserM2000SyaS,
issn = {0018-9219},
abstract = {This paper presents an account of the current state of sampling, 50 years after Shannon's formulation of the sampling theorem. The emphasis is on regular sampling, where the grid is uniform. This topic has benefitted from a strong research revival during the past few years, thanks in part to the mathematical connections that were made with wavelet theory. To introduce the reader to the modern, Hilbert-space formulation, we reinterpret Shannon's sampling procedure as an orthogonal projection onto the subspace of band-limited functions. We then extend the standard sampling paradigm for a presentation of functions in the more general class of "shift-in-variant" function spaces, including splines and wavelets. Practically, this allows for simpler-and possibly more realistic-interpolation models, which can be used in conjunction with a much wider class of (anti-aliasing) prefilters that are not necessarily ideal low-pass. We summarize and discuss the results available for the determination of the approximation error and of the sampling rate when the input of the system is essentially arbitrary; e.g., nonbandlimited. We also review variations of sampling that can be understood from the same unifying perspective. These include wavelets, multiwavelets, Papoulis generalized sampling, finite elements, and frames. Irregular sampling and radial basis functions are briefly mentioned.},
journal = {Proceedings of the IEEE},
pages = {569--587},
volume = {88},
publisher = {IEEE},
number = {4},
year = {2000},
title = {Sampling-50 years after Shannon},
copyright = {2000 INIST-CNRS},
language = {eng},
address = {New York, NY},
author = {Unser, M},
keywords = {Applied sciences ; Approximation error ; Exact sciences and technology ; Finite element methods ; Frequency ; Hilbert space ; Image reconstruction ; Information theory ; Information, signal and communications theory ; Interpolation ; Least squares approximation ; Sampling methods ; Sampling, quantization ; Signal and communications theory ; Signal sampling ; Telecommunications and information theory},
}

@article{Norton2008,
issn = {0007-0882},
abstract = {Constructivists, such as Harvey Brown, urge that the geometries of Newtonian and special relativistic spacetimes result from the properties of matter. Whatever this may mean, it commits constructivists to the claim that these spacetime geometries can be inferred from the properties of matter without recourse to spatiotemporal presumptions or with few of them. I argue that the construction project only succeeds if constructivists antecedently presume the essential commitments of a realist conception of spacetime. These commitments can be avoided only by adopting an extreme form of operationalism. <p><list list-type="order"><list-item><p>Introduction</p></list-item><list-item><p>The Construction Project</p></list-item><list-item><p>Clocks</p></list-item><list-item><p>The Spacetime Presumed</p></list-item><list-item><p>Lorentz Covariance Is a Property of a Matter Theory and Spacetime</p></list-item><list-item><p>Spatial Distances and Times Elapsed Are Properties of Spacetime</p></list-item><list-item><p>Conclusion</p></list-item></list></p>},
journal = {The British Journal for the Philosophy of Science},
pages = {821--834},
volume = {59},
publisher = {Oxford University Press},
number = {4},
year = {2008},
title = {{Why Constructive Relativity Fails}},
author = {Norton, John D.},
keywords = {Sciences (General) ; Philosophy;},
}

@article{BEH_2020,
   title={Bandlimited entanglement harvesting},
   volume={102},
   ISSN={2470-0029},
   url={http://dx.doi.org/10.1103/PhysRevD.102.125026},
   DOI={10.1103/physrevd.102.125026},
   number={12},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Henderson, Laura J. and Menicucci, Nicolas C.},
   year={2020},
   month={Dec} }

@article{UnsharpKempf,
   title={Fields over Unsharp Coordinates},
   volume={85},
   ISSN={1079-7114},
   url={http://dx.doi.org/10.1103/PhysRevLett.85.2873},
   DOI={10.1103/physrevlett.85.2873},
   number={14},
   journal={Physical Review Letters},
   publisher={American Physical Society (APS)},
   author={Kempf, Achim},
   year={2000},
   month={Oct},
   pages={2873–2876} }

@article{Kempf2013,
author = {Kempf,A.  and Chatwin-Davies,A.  and Martin,R. T. W. },
title = {A fully covariant information-theoretic ultraviolet cutoff for scalar fields in expanding Friedmann Robertson Walker spacetimes},
journal = {Journal of Mathematical Physics},
volume = {54},
number = {2},
pages = {022301},
year = {2013},
doi = {10.1063/1.4790482},

URL = { 
        https://doi.org/10.1063/1.4790482
    
},
eprint = { 
        https://doi.org/10.1063/1.4790482
    
}

}

@article{Pye2015,
   title={Locality and entanglement in bandlimited quantum field theory},
   volume={92},
   ISSN={1550-2368},
   url={http://dx.doi.org/10.1103/PhysRevD.92.105022},
   DOI={10.1103/physrevd.92.105022},
   number={10},
   journal={Physical Review D},
   publisher={American Physical Society (APS)},
   author={Pye, Jason and Donnelly, William and Kempf, Achim},
   year={2015},
   month={Nov} }

@misc{Pye2022,
    title={Lorentz-covariant sampling theory for fields},
    author={Pye, Jason},
    year={2022},
    eprint={2202.03589},
    archivePrefix={arXiv},
    primaryClass={hep-th},
    url={https://arxiv.org/abs/2202.03589}
}

@phdthesis{PyeThesis,
author={{Pye, Jason}},
title={On the Application of Bandlimitation and Sampling Theory to Quantum Field Theory},
year={2020},
school={University of Waterloo},
publisher="UWSpace",
url={http://hdl.handle.net/10012/16427}
}

@article{Kempf_2010,
	doi = {10.1088/1367-2630/12/11/115001},
	year = 2010,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {12},
	number = {11},
	pages = {115001},
	author = {Achim Kempf},
	title = {Spacetime could be simultaneously continuous and discrete, in the same way that information can be},
	journal = {New Journal of Physics},
	abstract = {There are competing schools of thought about the question of whether spacetime is fundamentally continuous or discrete. Here, we consider the possibility that spacetime could be simultaneously continuous and discrete, in the same mathematical way that information can be simultaneously continuous and discrete. The equivalence of continuous information and discrete information, which is of key importance in signal processing, is established by the Shannon sampling theory: for any band-limited signal, it suffices to record discrete samples to be able to perfectly reconstruct it everywhere, if the samples are taken at a rate of at least twice the band limit. It is known that physical fields on generic curved spaces obey a sampling theorem if they possess an ultraviolet cutoff. Most recently, methods of spectral geometry have been employed to show that also the very shape of a curved space (i.e. of a Riemannian manifold) can be discretely sampled and then reconstructed up to the cutoff scale. Here, we develop these results further and also consider the generalization to curved spacetimes, i.e. to Lorentzian manifolds.}
}

@article{Kempf_1997,
	doi = {10.1209/epl/i1997-00457-7},
	url = {https://doi.org/10.1209/epl/i1997-00457-7},
	year = 1997,
	month = {nov},
	publisher = {{IOP} Publishing},
	volume = {40},
	number = {3},
	pages = {257--262},
	author = {A Kempf},
	title = {On nonlocality, lattices and internal symmetries},
	journal = {Europhysics Letters ({EPL})},
	abstract = {We study functional analytic aspects of two types of correction terms to the Heisenberg algebra. One type of correction terms is known to induce a finite lower bound Δx0 to the resolution of distances, a short-distance cut-off which is motivated from string theory and quantum gravity. It implies the existence of families of lattices of position eigenvalues which form representations of certain unitary groups. Due to the finite Δx0 these lattices cannot be resolved on the given geometry. Within the framework, degrees of freedom that correspond to structure smaller than the resolvable (Planck) scale then turn into “internal” degrees of freedom with these unitary groups as symmetries. The other type of correction terms differs by a crucial sign and its basics are here considered for the first time.}
}

@article{ShannonOriginal,
author = {Shannon, C. E.},
title = {A Mathematical Theory of Communication},
year = {2001},
issue_date = {January 2001},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {5},
number = {1},
issn = {1559-1662},
url = {https://doi.org/10.1145/584091.584093},
doi = {10.1145/584091.584093},
journal = {SIGMOBILE Mob. Comput. Commun. Rev.},
month = {jan},
pages = {3–55},
numpages = {53}
}

@Article{Kempf2018,
author={Kempf, Achim},
title={Quantum Gravity, Information Theory and the CMB},
journal={Foundations of Physics},
year={2018},
month={Oct},
day={01},
volume={48},
number={10},
pages={1191-1203},
abstract={We review connections between the metric of spacetime and the quantum fluctuations of fields. We start with the finding that the spacetime metric can be expressed entirely in terms of the 2-point correlator of the fluctuations of quantum fields. We then discuss the open question whether the knowledge of only the spectra of the quantum fluctuations of fields also suffices to determine the spacetime metric. This question is of interest because spectra are geometric invariants and their quantization would, therefore, have the benefit of not requiring the modding out of diffeomorphisms. Further, we discuss the fact that spacetime at the Planck scale need not necessarily be either discrete or continuous. Instead, results from information theory show that spacetime may be simultaneously discrete and continuous in the same way that information can. Finally, we review the recent finding that a covariant natural ultraviolet cutoff at the Planck scale implies a signature in the cosmic microwave background (CMB) that may become observable.},
issn={1572-9516},
doi={10.1007/s10701-018-0163-2},
}

@article{Kempf2000b,
  title = {Unsharp degrees of freedom and the generating of symmetries},
  author = {Kempf, Achim},
  journal = {Phys. Rev. D},
  volume = {63},
  issue = {2},
  pages = {024017},
  numpages = {8},
  year = {2000},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.63.024017},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.63.024017}
}

@misc{Kempf2003,
	Archiveprefix = {arXiv},
	Author = {Kempf, Achim},
	Eprint = {0306104},
	Primaryclass = {gr-qc},
	Title = {{Aspects of Information Theory in Curved Space}},
	Year = {2003},
	url = {https://arxiv.org/abs/gr-qc/0306104}}
	
@article{Kempf2004a,
  title = {Covariant Information-Density Cutoff in Curved Space-Time},
  author = {Kempf, Achim},
  journal = {Phys. Rev. Lett.},
  volume = {92},
  issue = {22},
  pages = {221301},
  numpages = {4},
  year = {2004},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.92.221301},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.92.221301}
}

@article{Kempf2004b,
  title = {Fields with finite information density},
  author = {Kempf, Achim},
  journal = {Phys. Rev. D},
  volume = {69},
  issue = {12},
  pages = {124014},
  numpages = {15},
  year = {2004},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.69.124014},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.69.124014}
}



@inproceedings{Kempf2006,
	doi = {10.1142/9789812704030_0316},
  
	year = 2006,
	month = {feb},
  
	publisher = {World Scientific Publishing Company},
  
	author = {A. KEMPF},
  
	title = {{SHORT}-{DISTANCE} {CUTOFFS} {IN} {CURVED} {SPACE}
},
  
	booktitle = {The Tenth Marcel Grossmann Meeting}
}

@article{Menon2019,
issn = {0031-8248},
journal = {Philosophy of science},
pages = {1273--1283},
volume = {86},
publisher = {The University of Chicago Press},
number = {5},
year = {2019},
title = {{Algebraic Fields and the Dynamical Approach to Physical Geometry}},
copyright = {Copyright 2019 by the Philosophy of Science Association. All rights reserved.},
language = {eng},
address = {Cambridge},
author = {Menon, Tushar},
keywords = {Algebra ; Game theory ; Geometry ; Presumptions ; Relativity},
}



@Article{GelfandNaimark,
 Author = {Gelfand, I. and Naimark, M.},
 Title = {On the imbedding of normed rings into the ring of operators in {Hilbert} space},
 FJournal = {Matematicheski{\u{\i}} Sbornik. Novaya Seriya},
 Journal = {Mat. Sb., Nov. Ser.},
 Volume = {12},
 Pages = {197--213},
 Year = {1943},
 Language = {English},
 Keywords = {46L05},
 zbMATH = {3097323},
 Zbl = {0060.27006}
}

@Article{Geroch1972,
author={Geroch, Robert},
title={{Einstein Algebras}},
journal={Communications in Mathematical Physics},
year={1972},
month={12},
day={01},
volume={26},
number={4},
pages={271-275},
abstract={An approach to quantization of general relatively using a reformulation of the classical theory in which the events of space-time play essentially no role is discussed.},
issn={1432-0916},
doi={10.1007/BF01645521},
}

@article{Nonentity,
issn = {1871-1774},
journal = {Philosophy and Foundations of Physics},
volume = {1},
year = {2006},
title = {{Minkowski Space-Time: A Glorious Non-Entity}},
language = {eng},
author = {Brown, Harvey R. and Pooley, Oliver},
pages = {67-89},
}


@incollection{BrownPooley1999,
    author = {Brown, Harvey R. and Pooley, Oliver},
    title = {{The Origins of the Spacetime Metric: Bell’s {L}orentzian Pedagogy and its Significance in General Relativity}},
    publisher = {Cambridge University Press},
    booktitle = {Physics Meets Philosophy at the Planck Scale},
    editor = {Callender, Craig and Huggett, Nick},
    isbn = {052166280X},
    year = {2001},
    editors = {Callender, Craig and Huggett, Nick},
    chapter = {15},
    pages = {256--72},
}

@phdthesis{StevensSyman2014Tdat,
author = {Stevens, Syman},
title = {{The Dynamical Approach to Relativity as a Form of Regularity Relationalism}},
    school = {University of Oxford},
    year = {2014}
}

@article{TwiceOver,
issn = {0007-0882},
journal = {The British Journal for the Philosophy of Science},
pages = {837--878},
volume = {67},
publisher = {Oxford University Press},
number = {3},
year = {2016},
title = {Symmetry as an Epistemic Notion (Twice Over)},
author = {Dasgupta, Shamik},
keywords = {Sciences (General) ; Philosophy;},
}


@article{BelotGordon2000GaM,
issn = {00070882},
journal = {The British Journal for the Philosophy of Science},
pages = {561--595},
volume = {51},
publisher = {Oxford University Press},
year = {2000},
title = {Geometry and Motion},
language = {eng},
author = {Belot, Gordon},
keywords = {Physical sciences -- Physics -- Mechanics ; Physical sciences -- Astronomy -- Astrophysics ; Philosophy -- Metaphysics -- Cosmological philosophy ; Physical sciences -- Physics -- Theoretical physics ; Physical sciences -- Physics -- Theoretical physics ; Philosophy -- Metaphilosophy -- Natural philosophy ; Physical sciences -- Physics -- Theoretical physics ; Physical sciences -- Physics -- Geometry ; Mathematics -- Pure mathematics -- Statistics ; Mathematics -- Applied mathematics -- Statistics},
}

@article{HuggettNick2006TRAo,
issn = {0026-4423},
abstract = {A version of relationism that takes spatiotemporal structuresspatial geometry and a standard of inertiato supervene on the history of relations between bodies is described and defended. The account is used to explain how the relationist should construe models of Newtonian mechanics in which absolute acceleration manifestly does not supervene on the relations; Ptolemaic and Copernican models for example. The account introduces a new way in which a Lewis-style best system might capture regularities in a broadly Humean world; a defence is given against a charge of indeterminism that applies to any such approach to laws.},
journal = {Mind},
pages = {41--73},
volume = {115},
publisher = {Oxford University Press},
number = {457},
year = {2006},
title = {{The Regularity Account of Relational Spacetime}},
author = {Huggett, Nick},
keywords = {Spatial Analysis ; Time ; Philosophy;},
}

@incollection{Pooley2013,
publisher = {Oxford University Press},
booktitle = {The Oxford Handbook of Philosophy of Physics},
editor = {Batterman, Robert},
chapter = {15},
isbn = {9780195392043},
year = {2013},
title = {{Substantivalist and Relationalist Approaches to Spacetime}},
pages = {522-586},
language = {eng},
author = {Pooley, Oliver},
}

@article{DoratoMauro2007RTbS,
issn = {0269-8595},
journal = {International Studies in the Philosophy of Science},
pages = {95--102},
volume = {21},
publisher = {Routledge},
number = {1},
year = {2007},
title = {{Relativity Theory Between Structural and Dynamical Explanations}},
language = {eng},
author = {Dorato, Mauro},
keywords = {Sciences (General) ; Philosophy},
}

@misc{DiscreteGenCovPart2,
  doi = {10.48550/ARXIV.2205.07701},
  
  url = {https://arxiv.org/abs/2205.07701},
  
  author = {Grimmer, Daniel},
  
  keywords = {General Relativity and Quantum Cosmology (gr-qc), High Energy Physics - Lattice (hep-lat), History and Philosophy of Physics (physics.hist-ph), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {A Discrete Analog of General Covariance -- Part 2: Despite what you've heard, a perfectly Lorentzian lattice theory},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@ARTICLE{KempfDistCorr,
  
AUTHOR={Kempf, Achim},   
	 
TITLE={Replacing the Notion of Spacetime Distance by the Notion of Correlation},      
	
JOURNAL={Frontiers in Physics},      
	
VOLUME={9},      
	
YEAR={2021},      
	  
URL={https://www.frontiersin.org/article/10.3389/fphy.2021.655857},       
	
DOI={10.3389/fphy.2021.655857},      
	
ISSN={2296-424X},   
   
ABSTRACT={Spacetime is conventionally viewed as a stage on which actors, in the form of massive and massless matter, move. In this study, we explore what may lie beyond this picture. The starting point is the observation that quantum field fluctuations are the more strongly correlated the shorter their spacetime distance. The notion of spacetime distance can, therefore, be replaced by the notion of correlation strength. This suggests a new picture in which the abstract 2-point and multi-point correlations are the primary structure, a picture which is essentially information-theoretic. In the low energy regime, the secondary notions of spacetime and of matter would then emerge as approximate representations of the abstract correlators, namely, in the form of Feynman rules on curved spacetime.}
}

@article{ShapeFromSound,
  title = {Shape from Sound: Toward New Tools for Quantum Gravity},
  author = {Aasen, David and Bhamre, Tejal and Kempf, Achim},
  journal = {Phys. Rev. Lett.},
  volume = {110},
  issue = {12},
  pages = {121301},
  numpages = {5},
  year = {2013},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.110.121301},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.110.121301}
}

@misc{DiscreteGenCovPart1,
  doi = {10.48550/ARXIV.2204.02276},
  
  url = {https://arxiv.org/abs/2204.02276},
  
  author = {Grimmer, Daniel},
  
  keywords = {History and Philosophy of Physics (physics.hist-ph), General Relativity and Quantum Cosmology (gr-qc), High Energy Physics - Lattice (hep-lat), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {A Discrete Analog of General Covariance: Could the world be fundamentally set on a lattice?},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@incollection{Demarest2017,
publisher = {Oxford University Press},
booktitle = {Causal Powers},
isbn = {9780198796572},
year = {2017},
title = {{Powerful Properties, Powerless Laws}},
author = {Demarest, Heather},
editor = {Jonathan D. Jacobs},
chapter = {4},
pages = {38-54},
keywords = {Metaphysics ; Laws Of Nature ; Best System Account ; Fred Dretske ; David Lewis ; Barry Loewer ; Metaphysics},
}

@book{Lewis1973,
	author = {David Lewis},
	title = {Counterfactuals},
	year = {1973},
	publisher = {Blackwell Publishers}
}

@article{Lewis1994,
	volume = {103},
	journal = {Mind},
	number = {412},
	publisher = {Oxford University Press},
	title = {{Humean Supervenience Debugged}},
	year = {1994},
	author = {David Lewis},
	doi = {10.1093/mind/103.412.473},
	pages = {473--490}
}

@book{Lewis1999,
booktitle = {Papers in Metaphysics and Epistemology},
isbn = {9780511625343},
year = {1999},
title = {Papers in Metaphysics and Epistemology},
language = {eng},
publisher = {Cambridge University Press},
author = {Lewis, David},
keywords = {Metaphysics; Knowledge, Theory of},
}



@article{Cohen2009-COHABB,
	title = {A Better Best System Account of Lawhood},
	year = {2009},
	journal = {Philosophical Studies},
	volume = {145},
	number = {1},
	author = {Jonathan Cohen and Craig Callender},
	doi = {10.1007/s11098-009-9389-3},
	pages = {1--34},
	publisher = {Springer}
}

@article{BhogalHarjit2020Halo,
author = {Bhogal, Harjit},
title = {{Humeanism about Laws of Nature}},
journal = {Philosophy Compass},
volume = {15},
number = {8},
pages = {e12696},
issn = {1747-9991},
doi = {https://doi.org/10.1111/phc3.12696},
eprint = {https://compass.onlinelibrary.wiley.com/doi/pdf/10.1111/phc3.12696},
year = {2020}
}

@InCollection{sep-laws-of-nature,
	author       =	{Carroll, John W.},
	title        =	{{Laws of Nature}},
	booktitle    =	{The {Stanford} Encyclopedia of Philosophy},
	editor       =	{Edward N. Zalta},
	howpublished =	{\url{https://plato.stanford.edu/archives/win2020/entries/laws-of-nature/}},
	year         =	{2020},
	publisher    =	{Metaphysics Research Lab, Stanford University},
    address = {Stanford, CA},
}

@article{HempelCover,
 ISSN = {00318248, 1539767X},
 URL = {http://www.jstor.org/stable/185169},
 author = {Carl G. Hempel and Paul Oppenheim},
 journal = {Philosophy of Science},
 number = {2},
 pages = {135--175},
 publisher = {[The University of Chicago Press, Philosophy of Science Association]},
 title = {Studies in the Logic of Explanation},
 urldate = {2022-07-09},
 volume = {15},
 year = {1948}
}

@book{BirdTextbook,
    author = {Bird, Alexander},
    title = "{Nature's Metaphysics: Laws and Properties}",
    publisher = {Oxford University Press},
    address = {Oxford, UK},
    year = {2007},
    month = {06},
    isbn = {9780199227013},
    doi = {10.1093/acprof:oso/9780199227013.001.0001},
}

@article{LewisDavid1983Nwfa,
issn = {0004-8402},
journal = {Australasian journal of philosophy},
pages = {343--377},
volume = {61},
publisher = {Taylor & Francis Group},
number = {4},
year = {1983},
title = {{New Work for a Theory of Universals}},
language = {eng},
author = {Lewis, David},
keywords = {Philosophy},
}

@article{BusinessOfLaws,
issn = {0012-2017},
abstract = {Non‐Humean accounts of lawhood are said to founder on the Inference Problem, which is the problem of saying how laws that go beyond the regularities can entail the regularities. I argue that the Inference Problem has a simple solution – the Axiomatic Solution – on which the non‐Humean only needs to outfit her laws with a law‐to‐regularity axiom. There is a remaining Epistemic Bulge, as to why one should believe that the posit‐so‐axiomatized is to be found in nature, but the non‐Humean can flatten the bulge. Lawhood serves as a case study of how fundamental posits can do their business.},
journal = {Dialectica},
pages = {577--588},
volume = {70},
number = {4},
year = {2016},
title = {{It is the Business of Laws to Govern}},
author = {Schaffer, Jonathan},
keywords = {Philosophy;},
}

@book{RBrown2005,
	year = {2005},
	publisher = {Oxford University Press},
	title = {Physical Relativity: Space-Time Structure from a Dynamical Perspective},
	author = {Harvey R. Brown},
        address = {Oxford, UK},
}

@ARTICLE{Kempf2021,
AUTHOR={Kempf, Achim},   
TITLE={Replacing the Notion of Spacetime Distance by the Notion of Correlation},      
JOURNAL={Frontiers in Physics},      
VOLUME={9},           
YEAR={2021},      
URL={https://www.frontiersin.org/articles/10.3389/fphy.2021.655857},       
DOI={10.3389/fphy.2021.655857},      
ISSN={2296-424X},   
ABSTRACT={Spacetime is conventionally viewed as a stage on which actors, in the form of massive and massless matter, move. In this study, we explore what may lie beyond this picture. The starting point is the observation that quantum field fluctuations are the more strongly correlated the shorter their spacetime distance. The notion of spacetime distance can, therefore, be replaced by the notion of correlation strength. This suggests a new picture in which the abstract 2-point and multi-point correlations are the primary structure, a picture which is essentially information-theoretic. In the low energy regime, the secondary notions of spacetime and of matter would then emerge as approximate representations of the abstract correlators, namely, in the form of Feynman rules on curved spacetime.}
}

@book{MaudlinTim2012Pop:,
publisher = {Princeton University Press},
booktitle = {Philosophy of physics: {S}pace and time},
isbn = {9781400842339},
year = {2012},
title = {{Philosophy of Physics: Space and Time}},
author = {Maudlin, Tim},
keywords = {Space and time},
}


@incollection{BrownRead2018,
  author = {Harvey R. Brown and James Read},
  title     = {{The Dynamical Approach to Spacetime Theories}},
  booktitle = {The Routledge Companion to Philosophy of Physics},
  publisher = "Routledge",
  year      = {2022},
  editor    = {Knox, Eleanor and Wilson, Alastair},
  chapter   = {6},
  pages = {70-85},
}

@article{PhysRevD.95.024031,
  title = {Space from Hilbert space: Recovering geometry from bulk entanglement},
  author = {Cao, ChunJun and Carroll, Sean M. and Michalakis, Spyridon},
  journal = {Phys. Rev. D},
  volume = {95},
  issue = {2},
  pages = {024031},
  numpages = {20},
  year = {2017},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevD.95.024031},
  url = {https://link.aps.org/doi/10.1103/PhysRevD.95.024031}
}

@Article{GMostow2005,
author={Mostow, G. D.},
title={A Structure Theorem for Homogeneous Spaces},
journal={Geometriae Dedicata},
year={2005},
month={Aug},
day={01},
volume={114},
number={1},
pages={87-102},
abstract={A partial generalization of Sophus Lie's triangular form for solvable Lie algebras is presented. As application one is led to an iterated fibration for arbitrary homogeneous spaces. In the case of compact homogeneous spaces, one concludes easily that the Euler number is ≥0.},
issn={1572-9168},
doi={10.1007/s10711-004-1675-9},
url={https://doi.org/10.1007/s10711-004-1675-9}
}


@incollection{Hall2015,
author = {Hall, Ned},
publisher = {John Wiley and Sons, Ltd},
isbn = {9781118398593},
title = {{Humean Reductionism about Laws of Nature}},
booktitle = {A Companion to David Lewis},
chapter = {17},
pages = {262-277},
editor = {Loewer, Barry and Schaffer, Jonathan and Beebee, Helen},
doi = {https://doi.org/10.1002/9781118398593.ch17},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/9781118398593.ch17},
year = {2015},
keywords = {best system account (BSA), David Lewis, Humean reductionism, laws of nature, Newtonian particle world},
}

@misc{hokusai_1830,
title={{Under the Wave off {K}anagawa [Painting]}}, author={Hokusai, Katsushika}, year={1830}} 

@misc{Zikidis,
  author        = {Zikidis, Menelaos},
  title         = {Homogeneous Spaces: Characterization, construction and important examples},
  year          = {2016},
  publisher={Heidelberg University}
}

@article{GerochRobert1972Ea,
issn = {0010-3616},
journal = {Communications in mathematical physics},
pages = {271--275},
volume = {26},
publisher = {Springer-Verlag},
number = {4},
year = {1972},
title = {Einstein algebras},
copyright = {Copyright 1972 Springer-Verlag},
language = {eng},
author = {Geroch, Robert},
keywords = {83.22},
}

@phdthesis{jacobs2022a,
  year = {2022},
  edition = {},
  number = {},
  journal = {},
  pages = {},
  publisher = {University of Oxford},
  school = {University of Oxford},
  title = {Symmetries as a guide to the structure of physical quantities},
  volume = {},
  author = {Jacobs, C},
  editor = {},
  series = {}
}

@book{VanFraassenBasC.1980Tsie,
series = {Oxford scholarship online},
abstract = {Presenting an empiricist alternative to both logical positivism and scientific realism, this book insists on a literal understanding of the language of science and on an irreducibly pragmatic dimension of theory acceptance.},
publisher = {Clarendon},
booktitle = {The scientific image},
isbn = {9780191597473},
year = {1980},
title = {The scientific image},
language = {eng},
address = {Oxford},
author = {Van Fraassen, Bas C.},
keywords = {Science -- Philosophy; Empiricism},
}

@misc{Linnemann,
  doi = {10.48550/ARXIV.2112.09265},
  url = {https://arxiv.org/abs/2112.09265},
  author = {Linnemann, Niels and Salimkhani, Kian},
  keywords = {History and Philosophy of Physics (physics.hist-ph), FOS: Physical sciences, FOS: Physical sciences},
  title = {{The Constructivist's Programme and the Problem of Pregeometry}},
  publisher = {arXiv},
  year = {2021},
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@article{Chen_2021,
	doi = {10.1016/j.shpsa.2021.08.011},
	year = 2021,
	month = {8},
	publisher = {Elsevier {BV}},
	volume = {89},
	pages = {188--201},
	author = {Lu Chen and Tobias Fritz},
	title = {{An Algebraic Approach to Physical Fields}},
	journal = {Studies in History and Philosophy of Science Part A}
}

@article{ROSENSTOCK2015309,
title = {{On {E}instein Algebras and Relativistic Spacetimes}},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {52},
pages = {309-316},
year = {2015},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2015.09.003},
author = {Sarita Rosenstock and Thomas William Barrett and James Owen Weatherall},
keywords = {General relativity, Einstein algebras, Substantivalism, Relationism, Categorical equivalence},
abstract = {In this paper, we examine the relationship between general relativity and the theory of Einstein algebras. We show that according to a formal criterion for theoretical equivalence recently proposed by Halvorson, 2012, Halvorson, 2015 and Weatherall (2015a), the two are equivalent theories.}
}

@article{10.2307/188131,
 ISSN = {00318248, 1539767X},
 abstract = {In a number of publications, John Earman has advocated a tertium quid to the usual dichotomy between substantivalism and relationism concerning the nature of spacetime. The idea is that the structure common to the members of an equivalence class of substantival models is captured by a Leibniz algebra which can then be taken to directly characterize the intrinsic reality only indirectly represented by the substantival models. An alleged virtue of this is that, while a substantival interpretation of spacetime theories falls prey to radical local indeterminism, the Leibniz algebras do not. I argue that the program of Leibniz algebras is subject to radical local indeterminism to the same extent as substantivalism. In fact, for the category of topological spaces of interest in spacetime physics, the program is equivalent to the original spacetime approach. Moreover, the motivation for the program--that isomorphic substantival models should be regarded as representing the same physical situation--is misguided.},
 author = {Robert Rynasiewicz},
 journal = {Philosophy of Science},
 number = {4},
 pages = {572--589},
 publisher = {[The University of Chicago Press, Philosophy of Science Association]},
 title = {{Rings, Holes and Substantivalism: On the Program of {L}eibniz Algebras}},
 urldate = {2022-09-20},
 volume = {59},
 year = {1992}
}

@incollection{BrownHarveyR2013Etro,
    author = {Brown, Harvey R. and Lehmkuhl, Dennis},
    title = {{Einstein, the Reality of Space, and the Action-Reaction Principle}},
    booktitle = {Einstein, Tagore, and the Nature of Reality},
    editor = {Ghose, P},
    publisher = {Routledge},
    year = {2020}, 
    chapter = {1},
    pages = {1-20},
}

@article{DewarNeil2019GC,
issn = {0015-9018},
abstract = {This is an essay about general covariance, and what it says (or doesn’t say) about spacetime structure. After outlining a version of the dynamical approach to spacetime theories, and how it struggles to deal with generally covariant theories, I argue that we should think about the symmetry structure of spacetime rather differently in generally-covariant theories compared to non-generally-covariant theories: namely, as a form of internal rather than external symmetry structure.},
journal = {Foundations of physics},
pages = {294--318},
volume = {50},
publisher = {Springer US},
number = {4},
year = {2019},
title = {General-Relativistic Covariance},
copyright = {Springer Science+Business Media, LLC, part of Springer Nature 2019},
language = {eng},
address = {New York},
author = {Dewar, Neil},
keywords = {Classical and Quantum Gravitation ; Classical Mechanics ; Covariance ; History and Philosophical Foundations of Physics ; Philosophy of Science ; Physical Sciences ; Physics ; Physics and Astronomy ; Physics, Multidisciplinary ; Quantum Physics ; Relativity Theory ; Science & Technology ; Spacetime ; Special Issue : Hole Argument ; Statistical Physics and Dynamical Systems ; Symmetry},
}


@misc{LawsBeyondSpacetime,
  doi = {10.48550/ARXIV.2111.04500},
  
  url = {https://arxiv.org/abs/2111.04500},
  
  author = {Lam, Vincent and Wüthrich, Christian},
  
  keywords = {History and Philosophy of Physics (physics.hist-ph), General Relativity and Quantum Cosmology (gr-qc), FOS: Physical sciences, FOS: Physical sciences},
  
  title = {Laws beyond spacetime},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}

@article{knox2014spacetime,
  title={Spacetime structuralism or spacetime functionalism},
  author={Knox, Eleanor},
  journal={Manuscript. Unpublished draft available at https://www. eleanorknox. com/uploads/3/9/8/2/39826525/structuralism\_or\_functionalism\_draft\_2. pdf},
  year={2014}
}

@article{KNOX2019118,
title = {Physical relativity from a functionalist perspective},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {67},
pages = {118-124},
year = {2019},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2017.09.008},
author = {Eleanor Knox}
}

@article{KNOX2013346,
title = {Effective spacetime geometry},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {44},
number = {3},
pages = {346-356},
year = {2013},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2013.04.002},
url = {https://www.sciencedirect.com/science/article/pii/S1355219813000373},
author = {Eleanor Knox},
keywords = {Emergent spacetime, General relativity, Equivalence principle, Poincare gauge theory}
}

@article{Lam2020-LAMSFF,
	volume = {199},
	title = {Spacetime Functionalism From a Realist Perspective},
	year = {2020},
	doi = {10.1007/s11229-020-02642-y},
	author = {Vincent Lam and Christian W\"{u}thrich},
	pages = {1--19},
	publisher = {Springer},
	journal = {Synthese},
	number = {Suppl 2}
}

@article{LAM201839,
title = {Spacetime is as spacetime does},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {64},
pages = {39-51},
year = {2018},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2018.04.003},
url = {https://www.sciencedirect.com/science/article/pii/S1355219817301703},
author = {Vincent Lam and Christian Wüthrich},
keywords = {Emergence of spacetime, Functionalism, Empirical incoherence, Causal set theory, Loop quantum gravity, Local beables, Constitution, Multiple realizability},
abstract = {Theories of quantum gravity generically presuppose or predict that the reality underlying relativistic spacetimes they are describing is significantly non-spatiotemporal. On pain of empirical incoherence, approaches to quantum gravity must establish how relativistic spacetime emerges from their non-spatiotemporal structures. We argue that in order to secure this emergence, it is sufficient to establish that only those features of relativistic spacetimes functionally relevant in producing empirical evidence must be recovered. In order to complete this task, an account must be given of how the more fundamental structures instantiate these functional roles. We illustrate the general idea in the context of causal set theory and loop quantum gravity, two prominent approaches to quantum gravity.}
}

@book{Ott2022,
year = {2022},
title = {{The Metaphysics of Laws of Nature: {T}he Rules of the Game}},
language = {eng},
publisher = {Oxford University Press},
author = {Ott, Walter},
}

@book{ArmstrongNomNec,
place={Cambridge},
series={Cambridge Studies in Philosophy},
title={What is a Law of Nature?},
DOI={10.1017/CBO9781139171700},
publisher={Cambridge University Press},
author={Armstrong, David M.},
year={1983},
address={Cambridge, UK}
}

@article{LangeMarc2007Lamo,
issn = {1355-2198},
abstract = {Symmetry principles are commonly said to explain conservation laws—and were so employed even by Lagrange and Hamilton, long before Noether's theorem. But within a Hamiltonian framework, the conservation laws likewise entail the symmetries. Why, then, are symmetries explanatorily prior to conservation laws? I explain how the relation between ordinary (i.e., first-order) laws and the facts they govern (a relation involving counterfactuals) may be reproduced one level higher: as a relation between symmetries and the ordinary laws they govern. In that event, symmetries are
meta-laws; they are not mere
byproducts of the dynamical and force laws. Symmetries then explain conservation laws whereas conservation laws lack the modal status to explain symmetries. I elaborate the variety of natural necessity that meta-laws would possess. Proposed metaphysical accounts of natural law should aim to accommodate the distinction between meta-laws and mere byproducts of the laws just as they must accommodate the distinction between laws and accidents.},
journal = {Studies in History and Philosophy of Modern Physics},
pages = {457--481},
volume = {38},
publisher = {Elsevier Ltd},
number = {3},
year = {2007},
title = {Laws and meta-laws of nature: Conservation laws and symmetries},
copyright = {2006 Elsevier Ltd},
language = {eng},
author = {Lange, Marc},
keywords = {Conservation laws ; Counterfactuals ; Laws of nature ; Natural necessity ; Noether's theorem ; Symmetries},
}

@article{JANSSEN200926,
title = {{Drawing the Line between Kinematics and Dynamics in Special Relativity}},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {40},
number = {1},
pages = {26-52},
year = {2009},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2008.06.004},
author = {Michel Janssen},
keywords = {Lorentz invariance, Minkowski space–time, Kinematics, Trouton–Noble experiment, Classical electron models, Inference to the best explanation},
abstract = {Special relativity is preferable to those parts of Lorentz's classical ether theory it replaced because it shows that various phenomena that were given a dynamical explanation in Lorentz's theory are actually kinematical. In his book, Physical Relativity, Harvey Brown challenges this orthodox view. I defend it. The phenomena usually discussed in this context in the philosophical literature are length contraction and time dilation. I consider three other phenomena in the same class, each of which played a role in the early reception of special relativity in the physics literature: the Fresnel drag effect, the velocity dependence of electron mass, and the torques on a moving capacitor in the Trouton–Noble experiment. I offer historical sketches of how Lorentz's dynamical explanations of these phenomena came to be replaced by their now standard kinematical explanations. I then take up the philosophical challenge posed by the work of Harvey Brown and Oliver Pooley and clarify how those kinematical explanations work. In the process, I draw attention to the broader importance of the kinematics–dynamics distinction.}
}

@incollection{Ott2009,
    author = {Ott, Walter},
    isbn = {9780199570430},
    title = "{Occasionalism}",
    chapter = {9},
    pages = {64-78},
    booktitle = "{Causation and Laws of Nature in Early Modern Philosophy}",
    publisher = {Oxford University Press},
    year = {2009},
    month = {09},
    abstract = "{The top‐down nature of Descartes's view commits him to occasionalism, at least where body–body causation is concerned. This chapter rounds out the argument for this reading, appealing chiefly to the laws of nature: given their status as divine commands, Cartesian laws must be implemented at every moment by God himself. There is no sense to be made of the laws operating independently of God's activity. This reading is then defended against the concurrentist interpretation of Descartes.}",
    doi = {10.1093/acprof:oso/9780199570430.003.0010},
    eprint = {https://academic.oup.com/book/0/chapter/290816460/chapter-ag-pdf/44521609/book\_34299\_section\_290816460.ag.pdf},
}

@article{Curiel2020,
year = {2020},
title = {{Schematizing the Observer and the Epistemic Content of Theories}},
copyright = {http://arxiv.org/licenses/nonexclusive-distrib/1.0},
language = {eng},
author = {Curiel, Erik},
keywords = {Physics - History and Philosophy of Physics},
journal={arXiv preprint arXiv:1903.02182},
}

@book{KantCritiqueOfPureReason,
series = {Everyman's library},
publisher = {J.M. Dent ; E.P. Dutton},
year = {1946},
title = {Critique of pure reason},
language = {eng},
address = {London : New York},
author = {Kant, Immanuel},
}

@book{MalamentTopics,
series = {Chicago lectures in physics},
publisher = {University of Chicago Press},
booktitle = {Topics in the foundations of general relativity and Newtonian gravitation theory},
year = {2012},
title = {Topics in the foundations of general relativity and Newtonian gravitation theory},
language = {eng},
address = {Chicago ; London},
author = {Malament, David B},
keywords = {Relativity (Physics); Gravitation},
}

@article{le_bihan_duality_2018,
	title = {Duality and ontology},
	volume = {13},
	url = {https://doi.org/10.1111/phc3.12555},
	abstract = {Abstract A ?duality? is a formal mapping between the spaces of solutions of two empirically equivalent theories. In recent times, dualities have been found to be pervasive in string theory and quantum field theory. Naïvely interpreted, duality-related theories appear to make very different ontological claims about the world?differing in, for example, spacetime structure, fundamental ontology, and mereological structure. In light of this, duality-related theories raise questions familiar from discussions of underdetermination in the philosophy of science: in the presence of dual theories, what is one to say about the ontology of the world? In this paper, we undertake a comprehensive and nontechnical survey of the landscape of possible ontological interpretations of duality-related theories. We provide a significantly enriched and clarified taxonomy of options?several of which are novel to the literature.},
	pages = {e12555},
	number = {12},
	journaltitle = {Philosophy Compass},
	shortjournal = {Philosophy Compass},
	author = {Le Bihan, Baptiste and Read, James},
	urldate = {2019-01-11},
	date = {2018-12-01},
 year = {2018}
}

@misc{pittphilsci19993,
           month = {December},
           title = {Philosophy, physics, and the problems of spacetime emergence},
          author = {Rasmus Jaksland and Kian Salimkhani},
            year = {2021},
        keywords = {Spacetime Emergence, Spacetime, Quantum Gravity, Metaphysics of Science},
             url = {http://philsci-archive.pitt.edu/19993/},
}

﻿@Article{LeBihan2021,
author={Le Bihan, Baptiste},
title={Spacetime emergence in quantum gravity: functionalism and the hard problem},
journal={Synthese},
year={2021},
month={Dec},
day={01},
volume={199},
number={2},
pages={371-393},
abstract={Spacetime functionalism is the view that spacetime is a functional structure implemented by a more fundamental ontology. Lam and W{\"u}thrich have recently argued that spacetime functionalism helps to solve the epistemological problem of empirical coherence in quantum gravity and suggested that it also (dis)solves the hard problem of spacetime, namely the problem of offering a picture consistent with the emergence of spacetime from a non-spatio-temporal structure. First, I will deny that spacetime functionalism solves the hard problem by showing that it comes in various species, each entailing a different attitude towards, or answer to, the hard problem. Second, I will argue that the existence of an explanatory gap, which grounds the hard problem, has not been correctly taken into account in the literature.},
issn={1573-0964},
doi={10.1007/s11229-019-02449-6},
url={https://doi.org/10.1007/s11229-019-02449-6}
}

@article{MaudlinEssence,
 ISSN = {02708647},
 URL = {http://www.jstor.org/stable/192873},
 abstract = {I argue that Norton & Earman's hole argument, despite its historical association with General Relativity, turns upon very general features of any linguistic system that can represent substances by names. After exploring various means by which mathematical objects can be interpreted as representing physical possibilities, I suggest that a form of essentialism can solve the hole dilemma without abandoning either determinism or substantivalism. Finally, I identify the basic tenets of such an essentialism in Newton's writings and consider how they can be updated to apply to the case provided by General Relativity.},
 author = {Tim Maudlin},
 journal = {PSA: Proceedings of the Biennial Meeting of the Philosophy of Science Association},
 number = {},
 pages = {82--91},
 publisher = {[University of Chicago Press, Springer, Philosophy of Science Association]},
 title = {The Essence of Space-Time},
 urldate = {2023-03-02},
 volume = {1988},
 year = {1988}
}

@article{RichardEdu,
  title = {Dimensional reduction of cavities with axial symmetry: A complete analysis of when an optical fiber is approximately one dimensional},
  author = {Grimmer, Daniel and Lopp, Richard and Mart\'{\i}n-Mart\'{\i}nez, Eduardo},
  journal = {Phys. Rev. A},
  volume = {104},
  issue = {1},
  pages = {013723},
  numpages = {13},
  year = {2021},
  month = {Jul},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevA.104.013723},
  url = {https://link.aps.org/doi/10.1103/PhysRevA.104.013723}
}

@article{Weyl1911,
author = {Weyl, H.},
journal = {Nachrichten von der Gesellschaft der Wissenschaften zu Göttingen, Mathematisch-Physikalische Klasse},
pages = {110-117},
title = {\"Ueber die asymptotische Verteilung der Eigenwerte},
volume = {1911},
year = {1911},
}

@Article{Weyl1912,
author={Weyl, Hermann},
title={Das asymptotische Verteilungsgesetz der Eigenwerte linearer partieller Differentialgleichungen (mit einer Anwendung auf die Theorie der Hohlraumstrahlung)},
journal={Math. Ann.},
year={1912},
volume={71},
number={4},
pages={441-479},
doi={10.1007/BF01456804}
}

@book{IntroToLieGeoHomo,
series = {Student mathematical library. v. 22},
publisher = {American Mathematical Society},
isbn = {9780821827789},
year = {2003},
title = {An introduction to Lie groups and the geometry of homogeneous spaces},
language = {eng},
address = {Providence, RI},
author = {Arvanitogeōrgos, Andreas},
keywords = {Lie groups; Homogeneous spaces},
lccn = {2003058352},
}

@book{WarnerFrankW1983Fodm,
series = {Graduate texts in mathematics ; 94},
booktitle = {Foundations of differentiable manifolds and Lie groups},
isbn = {9781475717990 (electronic bk.)},
year = {1983},
title = {Foundations of differentiable manifolds and Lie groups},
publisher={Springer},
language = {eng},
address = {New York},
author = {Warner, Frank W},
keywords = {Differentiable manifolds; Lie groups; Variétés différentiables; Lie, Groupes de; Differentiable manifolds; Lie groups; Manifolds; Differentieerbaarheid; Lie-groepen; Variétés différentielles; Lie, groupes de},
}

@book{BrickellF1970Dm:a,
series = {New university mathematics series},
publisher = {Van Nostrand Reinhold},
isbn = {9780442010485},
year = {1970},
title = {Differentiable manifolds: an introduction},
language = {eng},
address = {London},
author = {Brickell, F and Clark, Ronald Sydney},
keywords = {Differentiable manifolds},
lccn = {LC},
}

@book{KobayashiShoshichi1996Fodg,
series = {Wiley classics library},
publisher = {Wiley},
isbn = {9780471157335},
year = {1996},
title = {Foundations of differential geometry},
language = {eng},
address = {New York ; Chichester},
author = {Kobayashi, Shoshichi and Nomizu, Katsumi},
keywords = {Geometry, Differential},
}

﻿@Article{Bain2013,
author={Bain, Jonathan},
title={Category-theoretic structure and radical ontic structural realism},
journal={Synthese},
year={2013},
month={Jun},
day={01},
volume={190},
number={9},
pages={1621-1635},
abstract={Radical ontic structural realism (ROSR) claims that structure exists independently of objects that may instantiate it. Critics of ROSR contend that this claim is conceptually incoherent, insofar as, (i) it entails there can be relations without relata, and (ii) there is a conceptual dependence between relations and relata. In this essay I suggest that (ii) is motivated by a set-theoretic formulation of structure, and that adopting a category-theoretic formulation may provide ROSR with more support. In particular, I consider how a category-theoretic formulation of structure can be developed that denies (ii), and can be made to do work in the context of formulating theories in physics.},
issn={1573-0964},
doi={10.1007/s11229-011-9896-6},
url={https://doi.org/10.1007/s11229-011-9896-6}
}

@misc{ConnesSpectralGeometry,
  doi = {10.48550/ARXIV.0810.2088},
  
  url = {https://arxiv.org/abs/0810.2088},
  
  author = {Connes, Alain},
  
  keywords = {Operator Algebras (math.OA), High Energy Physics - Theory (hep-th), Quantum Algebra (math.QA), FOS: Mathematics, FOS: Mathematics, FOS: Physical sciences, FOS: Physical sciences, 46L87; 58B34},
  
  title = {On the spectral characterization of manifolds},
  
  publisher = {arXiv},
  
  year = {2008},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{Kempf2008,
  title = {Information Theory, Spectral Geometry, and Quantum Gravity},
  author = {Kempf, Achim and Martin, Robert},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {2},
  pages = {021304},
  numpages = {4},
  year = {2008},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.100.021304},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.100.021304}
}

@article{Rynasiewicz,
 ISSN = {00318248, 1539767X},
 abstract = {In a number of publications, John Earman has advocated a tertium quid to the usual dichotomy between substantivalism and relationism concerning the nature of spacetime. The idea is that the structure common to the members of an equivalence class of substantival models is captured by a Leibniz algebra which can then be taken to directly characterize the intrinsic reality only indirectly represented by the substantival models. An alleged virtue of this is that, while a substantival interpretation of spacetime theories falls prey to radical local indeterminism, the Leibniz algebras do not. I argue that the program of Leibniz algebras is subject to radical local indeterminism to the same extent as substantivalism. In fact, for the category of topological spaces of interest in spacetime physics, the program is equivalent to the original spacetime approach. Moreover, the motivation for the program--that isomorphic substantival models should be regarded as representing the same physical situation--is misguided.},
 author = {Robert Rynasiewicz},
 journal = {Philosophy of Science},
 number = {4},
 pages = {572--589},
 publisher = {[The University of Chicago Press, Philosophy of Science Association]},
 title = {Rings, Holes and Substantivalism: On the Program of {L}eibniz Algebras},
 urldate = {2022-09-20},
 volume = {59},
 year = {1992}
}

﻿@Article{Beem1991,
author={Beem, John K.
and Parker, Phillip E.},
title={The space of geodesics},
journal={Geometriae Dedicata},
year={1991},
month={Apr},
day={01},
volume={38},
number={1},
pages={87-99},
issn={1572-9168},
doi={10.1007/BF00147737},
}

@book{NewtonPrincipia,
series = {Ebook central},
booktitle = {The principia: mathematical principles of natural philosophy},
isbn = {9780520964785},
year = {1999},
title = {The principia: mathematical principles of natural philosophy},
language = {eng},
address = {Oakland, California},
author = {Newton, Isaac},
keywords = {Newton, Isaac, 1642-1727. Principia; Mechanics -- Early works to 1800; Celestial mechanics -- Early works to 1800},
}

@InCollection{sep-spacetime-theories-classical,
	author       =	{Hoefer, Carl and Huggett, Nick and Read, James},
	title        =	{{Absolute and Relational Space and Motion: Classical Theories}},
	booktitle    =	{The {Stanford} Encyclopedia of Philosophy},
	editor       =	{Edward N. Zalta and Uri Nodelman},
	howpublished =	{\url{https://plato.stanford.edu/archives/spr2023/entries/spacetime-theories-classical/}},
	year         =	{2023},
	edition      =	{{S}pring 2023},
	publisher    =	{Metaphysics Research Lab, Stanford University}
}

@InCollection{sep-spacetime-theories,
	author       =	{Huggett, Nick and Hoefer, Carl and Read, James},
	title        =	{{Absolute and Relational Space and Motion: Post-Newtonian Theories}},
	booktitle    =	{The {Stanford} Encyclopedia of Philosophy},
	editor       =	{Edward N. Zalta and Uri Nodelman},
	howpublished =	{\url{https://plato.stanford.edu/archives/sum2023/entries/spacetime-theories/}},
	year         =	{2023},
	edition      =	{{S}ummer 2023},
	publisher    =	{Metaphysics Research Lab, Stanford University}
}

@article{BH2016,
issn = {1755-0203},
abstract = {Abstract Logicians and philosophers of science have proposed various formal criteria for theoretical equivalence. In this paper, we examine two such proposals: definitional equivalence and categorical equivalence. In order to show precisely how these two well-known criteria are related to one another, we investigate an intermediate criterion called Morita equivalence.},
pages = {556--582},
volume = {9},
journal = {The Review of Symbolic Logic},
publisher = {Cambridge University Press},
number = {3},
year = {2016},
title = {{Morita Equivalence}},
author = {Barrett, Thomas William and Halvorson, Hans},
keywords = {Mathematics - Logic ; Mathematics - Category Theory ; Physics - History And Philosophy Of Physics;},
}

@book{QuineW.V1948Owti,
publisher = {[Catholic University of America, Philosophy Education Society]},
booktitle = {On what there is},
year = {1948},
title = {On what there is.},
language = {eng},
address = {Washington, D.C.},
author = {Quine, W. V},
keywords = {Ontology},
}

@Book{BourbakiTopology,
author={Bourbaki, N.},
title={General Topology: Chapters 1-4},
year={2013},
month={Dec},
day={01 ER - },
publisher={Springer},
isbn={9783642617010}
}

@book{TopologicalTransformations,
publisher = {Interscience Publishers},
year = {1955},
title = {Topological transformation groups [by] Deane Montgomery [and] Leo Zippin},
language = {eng},
address = {New York (State)},
author = {Montgomery, Deane, 1909-1992},
}

@article{ArensHomeoGroup,
 ISSN = {00029327, 10806377},
 URL = {http://www.jstor.org/stable/2371787},
 author = {Richard Arens},
 journal = {American Journal of Mathematics},
 number = {4},
 pages = {593--610},
 publisher = {Johns Hopkins University Press},
 title = {Topologies for Homeomorphism Groups},
 urldate = {2023-07-17},
 volume = {68},
 year = {1946}
}

@article{IntroISE,
    title={{{\GG{1}} {I}ntroducing the {ISE M}ethodology: A Powerful New Tool for Topological Redescription}},
    author={Daniel Grimmer},
    year={2023},
   journal={arXiv preprint arXiv:2303.04130},
}

@article{ISEEquiv,
      title={{{\GG{2}} {I}n Search of New Spacetimes: Topological Redescription and the {ISE}-Equivalence Theorem}}, 
      author={Daniel Grimmer},
      year={2023},
      journal={arXiv preprint arXiv:2306.08110},
}

@article{IntroISE-Blind,
    title={{{\GG{1}} Omitted for Peer Review}},
    author={Omitted},
    year={2023},
}

@article{ISEEquiv-Blind,
    title={{{\GG{2}} Omitted for Peer Review}},
    author={Omitted},
    year={2023},
}

@incollection{ExplainUnify,
	editor = {Philip Kitcher and Wesley Salmon},
	year = {1989},
	title = {{Explanatory Unification and the Causal Structure of the World}},
	author = {Philip Kitcher},
	booktitle = {Scientific Explanation},
	publisher = {University of Minnesota Press},
	pages = {410--505}
}


@incollection{KantDissertation,
place={Cambridge},
title={{On The Form And Principles Of The Sensible And The Intelligible World [Inaugural Dissertation] (1770)}},
booktitle={Theoretical Philosophy, 1755–1770},
publisher={Cambridge University Press},
author={Kant, Immanuel},
editor={Walford, David and Meerbote, Ralf},
year={1992}, 
pages={373–416}, 
collection={The Cambridge Edition of the Works of Immanuel Kant} 
}

@article{STepistemology,
author = {Dewar, Neil and Linnemann, Niels and Read, James},
title = {{The Epistemology of Spacetime}},
journal = {Philosophy Compass},
volume = {17},
number = {4},
pages = {e12821},
doi = {https://doi.org/10.1111/phc3.12821},
eprint = {https://compass.onlinelibrary.wiley.com/doi/pdf/10.1111/phc3.12821},
abstract = {Abstract How is it that the basic structures of space and time come to manifest themselves in physical theories and theorising, and in our empirical experience of the world? This question is central to an important field of the philosophy of physics: the epistemology of spacetime. In this article, we survey systematically the various responses which have been offered to this question, highlighting little-explored connections and open research questions.},
year = {2022}
}

@book{Poincare,
publisher = {Bloomsbury Publishing},
booktitle = {Science and Hypothesis},
isbn = {9781350026780},
year = {2018},
title = {Science and Hypothesis: The Complete Text},
language = {eng},
author = {Poincaré, Henri},
keywords = {conventions ; electrodynamics ; Epistemology ; ether theories ; Hypotheses ; mathematical induction ; mechanics ; non-Euclidean geometry ; Philosophy ; Philosophy of Mathematics and Logic ; Philosophy of Science ; probabilities ; Science ; thermodynamics},
}

@article{pittphilsci8895,
title = {{The Nontriviality of Trivial General Covariance: How Electrons Restrict ‘Time’ Coordinates, Spinors (Almost) Fit into Tensor Calculus, and 7/16 of a Tetrad is Surplus Structure}},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {43},
number = {1},
pages = {1-24},
year = {2012},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2011.11.001},
author = {Brian Pitts},

}

@article{Acuna2016,
title = {Minkowski {S}pacetime and {L}orentz {I}nvariance: The {C}art and the {H}orse or {T}wo {S}ides of a {S}ingle {C}oin?},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {55},
pages = {1-12},
year = {2016},
author = {Pablo Acuña},
keywords = {Lorentz invariance, Minkowski spacetime, Explanation, Theories of principle, Constructive theories, Spacetime ontology},
}

@article{linnemann2021constructivists,
      title={The Constructivist's Programme and the Problem of Pregeometry}, 
      author={Niels Linnemann and Kian Salimkhani},
      year={2021},
      journal={arXiv preprint arXiv:2112.09265},
}

@article{IVANOVA2015114,
title = {{Conventionalism, structuralism and neo-{K}antianism in {P}oincaré's philosophy of science}},
journal = {Studies in History and Philosophy of Science Part B: Studies in History and Philosophy of Modern Physics},
volume = {52},
pages = {114-122},
year = {2015},
issn = {1355-2198},
doi = {https://doi.org/10.1016/j.shpsb.2015.03.003},
author = {Milena Ivanova},
keywords = {Conventionalism, Henri Poincaré, Neo-Kantianism, Structural realism, Synthetic }
}

@book{read_2023,
place={Cambridge},
series={Elements in the Philosophy of Physics},
title={Special Relativity},
DOI={10.1017/9781009300599},
publisher={Cambridge University Press},
author={Read, James},
year={2023},
collection={Elements in the Philosophy of Physics}}

@incollection{Halvorson2016,
	author = {Hans Halvorson},
	booktitle = {The Oxford Handbook of Philosophy of Science},
	year = {2016},
	title = {{Scientific Theories}},
	pages = {585--608},
        chapter = {28},
	editor = {Paul Humphreys},
	publisher = {Oxford University Press}
}

@article{pittphilsci19728,
	author = {David Wallace},
	doi = {10.1016/j.shpsa.2022.01.015},
	journal = {Studies in History and Philosophy of Science Part A},
	number = {C},
	pages = {239--248},
	title = {{Isolated Systems and Their Symmetries, Part {I}: General Framework and Particle-Mechanics Examples}},
	volume = {92},
	year = {2022}
}


@book{PlatoMeno,
booktitle = {Meno},
isbn = {9781603847872 (electronic bk.)},
year = {1980},
title = {Meno},
language = {eng},
author = {Plato},
editor = {Grube, G. M. A},
publisher = {Hackett Publishing Company},
}

@book{Plato1997Cwer,
booktitle = {Complete Works},
isbn = {9781603846707},
year = {1997},
title = {Complete works},
language = {eng},
author = {Plato},
editor = {Cooper, John M and Hutchinson, D. S.},
publisher = {Hackett Publishing Company},
keywords = {Socrates; Philosophy, Ancient},
}

@book{Lewis1986,
    author = {Lewis, David},
    title = "{Philosophical Papers Volume II}",
    publisher = {Oxford University Press},
    year = {1986},
    month = {06},
    isbn = {9780195036466},
    doi = {10.1093/0195036468.001.0001},
    url = {https://doi.org/10.1093/0195036468.001.0001},
}

@book{HumeText,
keywords = {Knowledge, Theory of -- Early works to 1800},
language = {eng},
publisher = {Oxford University Press},
series = {Oxford world's classics},
title = {An enquiry concerning human understanding },
year = {2020},
booktitle = {An enquiry concerning human understanding},
abstract = {David Hume (1711-1776) is thought to be one of the greatest philosophers. In this text, Hume gives an accessible presentation of strikingly original and challenging views concerning human understanding.},
author = {Hume, David and Millican, P. J. R.},
address = {Oxford},
edition = {New edition / edited with an introduction and notes by Peter Millican.},
isbn = {0-19-192173-4},
}

@incollection{TwoHumeReadings,
    author = {Lorkowski, C. M.},
    title = {David {H}ume: Causation},
    booktitle = {The Internet Encyclopedia of Philosophy},
    publisher = {The Internet Encyclopedia of Philosophy},
    year = {2023},
    issn = {2161-0002},
}

@book{ThirdHumeReading,
  title={The Philosophy of David Hume: With a New Introduction by Don Garrett},
  author={Smith, N.K.},
  isbn={9780230511170},
  year={2005},
  publisher={Palgrave Macmillan UK}
}

@inbook{Mentaculus,
author = { Barry   Loewer },
title = {The Mentaculus Vision},
year = {2020},
booktitle = {Statistical Mechanics and Scientific Explanation},
chapter = {Chapter 1},
publisher = {World Scientific},
pages = {3-29},
doi = {10.1142/9789811211720_0001},
}

@Article{PackageDeal,
author={Loewer, Barry},
title={The package deal account of laws and properties (PDA)},
journal={Synthese},
year={2021},
month={Dec},
day={01},
volume={199},
number={1},
pages={1065-1089},
issn={1573-0964},
doi={10.1007/s11229-020-02765-2},
url={https://doi.org/10.1007/s11229-020-02765-2}
}

@book{AfterPhysics,
author = {Albert, David Z.},
address = {Cambridge},
booktitle = {After physics},
isbn = {9780674731264},
keywords = {Physics -- Philosophy},
language = {eng},
publisher = {Harvard University Press},
title = {After physics },
year = {2015},
}

@article{Abraham1912,
    author = {Abraham, Max},
    title = {Zur Theorie der Gravitation},
    journal = {Physikalische Zeitschrift},
    year = {1912},
    volume = {13},
    pages = {1-4},
}

@article{Nordstrom1,
    author = {Nordstr\"{o}m, Gunnar },
    title = {Relativitätsprinzip und Gravitation},
    journal = {Physikalische Zeitschrift},
    year = {1912},
    volume = {13},
    pages = {1126-1129},
}

@article{Nordstrom2,
    author = {Nordstr\"{o}m, Gunnar},
    title = {Zur theorie der Gravitation vom standpunkt der Relativitätsprinzips},
    journal = {Annalen der Physik},
    year = {1913},
    volume = {42},
    pages = {533-554},
}

@book{SchopenhauerV2,
author = {Schopenhauer, Arthur and Norman, Judith and Janaway, Christopher and Welchman, Alistair},
address = {Cambridge ;},
booktitle = {The world as will and representation. Volume 2},
isbn = {1-108-57836-5},
keywords = {Philosophy},
language = {eng},
publisher = {Cambridge University Press},
series = {The Cambridge edition of the works of Schopenhauer},
title = {The world as will and representation. Volume 2 },
year = {2018},
}

@article{EmpiricalIncoherence,
author = {Huggett, Nick and Wüthrich, Christian},
copyright = {2012 Elsevier Ltd},
issn = {1355-2198},
journal = {Studies in History and Philosophy of Modern Physics},
keywords = {Quantum gravity},
language = {eng},
number = {3},
pages = {276-285},
publisher = {Elsevier Ltd},
title = {Emergent spacetime and empirical (in)coherence},
volume = {44},
year = {2013},
}

@article{Blackburn1990,
author = {Blackburn, Simon},
address = {Buffalo, N.Y},
language = {eng},
pages = {237-250},
publisher = {Brown University},
title = {Hume and Thick Connexions},
volume = {50},
year = {1990},
}

@book{Prolegomena,
author = {Kant, Immanuel and Hatfield, Gary C.},
address = {Cambridge, UK ;},
booktitle = {Prolegomena to any future metaphysics that will be able to come forward as science : with selections from the Critique of pure reason},
edition = {Rev. ed.},
isbn = {0511184832},
keywords = {Connaissance, Théorie de la},
language = {eng},
publisher = {Cambridge University Press},
series = {Cambridge texts in the history of philosophy},
title = {Prolegomena to any future metaphysics that will be able to come forward as science : with selections from the Critique of pure reason },
year = {2004},
}

@book{WaldGR,
author = {Wald, Robert M.},
address = {Chicago ;},
booktitle = {General relativity},
isbn = {0226870324},
keywords = {General relativity (Physics)},
language = {eng},
publisher = {University of Chicago Press},
title = {General relativity },
year = {1984},
}

@book{Carroll1994,
	address = {Cambridge, UK},
	author = {John W. Carroll},
	editor = {},
	publisher = {Cambridge University Press},
        title = {Laws of Nature},
	year = {1994}
}

@incollection{MaudlinPrimitiveLaws,
author = {Maudlin, Tim},
address = {United Kingdom},
booktitle = {The Metaphysics Within Physics},
isbn = {9780199218219},
keywords = {Physics},
language = {eng},
publisher = {Oxford University Press},
title = {A Modest Proposal Concerning Laws, Counterfactuals, and Explanations},
year = {2007},
}

@article{Dretske1977,
	author = {Fred I. Dretske},
	doi = {10.1086/288741},
	journal = {Philosophy of Science},
	number = {2},
	pages = {248--268},
	publisher = {University of Chicago Press},
	title = {Laws of Nature},
	volume = {44},
	year = {1977}
}

@article{Tooley1977,
	author = {Michael Tooley},
	doi = {10.1080/00455091.1977.10716190},
	journal = {Canadian Journal of Philosophy},
	number = {4},
	pages = {667--98},
	publisher = {University of Calgary Press},
	title = {The Nature of Laws},
	volume = {7},
	year = {1977}
}

@incollection{Psillos2018,
    author = {Psillos, Stathis},
    isbn = {9780198746775},
    title = {Laws and Powers in the Frame of Nature},
    booktitle = {Laws of Nature},
    publisher = {Oxford University Press},
    year = {2018},
    month = {05},
    doi = {10.1093/oso/9780198746775.003.0005},
    url = {https://doi.org/10.1093/oso/9780198746775.003.0005},
    eprint = {https://academic.oup.com/book/0/chapter/153720326/chapter-ag-pdf/44963787/book\_8193\_section\_153720326.ag.pdf},
}

@phdthesis{GrimmerThesis,
author={Grimmer, Daniel},
title={Searching for New Spacetimes: Towards a Dynamics-First View of Topology},
year={2024},
school={University of Oxford},
address = {Oxford, UK}
}

@phdthesis{OmittedThesis,
author={Omitted, Omitted},
title={Omitted for Peer-Review},
year={2024},
}

@article{DewarInternal,
	author = {Neil Dewar},
	doi = {10.1007/s11229-023-04102-9},
	journal = {Synthese},
	number = {4},
	pages = {1--24},
	publisher = {Springer Verlag},
	title = {Interpretation and Equivalence; or, Equivalence and Interpretation},
	volume = {201},
	year = {2023}
}

@book{DewarBook,
	author = {Neil Dewar},
	editor = {},
	publisher = {Cambridge University Press},
	title = {Structure and Equivalence},
	year = {2022},
        address = {Cambridge, UK}
}

@book{NaturalGaugeNatural,
  title={Natural and Gauge Natural Formalism for Classical Field Theorie: A Geometric Perspective including Spinors and Gauge Theories},
  author={Fatibene, L. and Francaviglia, M.},
  isbn={9781402017032},
  lccn={03064183},
  year={2003},
  publisher={Springer},
  address={Dordrecht, NL}
}

@article{RasmusEnrico,
author = {Grimmer, Daniel and Cinti, Enrico and Jaksland, Rasmus},
title = {Duality, Underdetermination, and the Uncommon Common Core},
journal = {The British Journal for the Philosophy of Science},
volume = {0},
number = {ja},
pages = {null},
year = {2024},
doi = {10.1086/730421},
eprint = { https://doi.org/10.1086/730421}
}

@Article{DeHaro2021,
author={De Haro, Sebastian
and Butterfield, Jeremy},
title={{On Symmetry and Duality}},
journal={Synthese},
year={2021},
month={Apr},
day={01},
volume={198},
number={4},
pages={2973-3013},
abstract={We advocate an account of dualities between physical theories: the basic idea is that dual theories are isomorphic representations of a common core. We defend and illustrate this account, which we call a Schema, in relation to symmetries. Overall, the account meshes well with standard treatments of symmetries. But the distinction between the common core and the dual theories prompts a distinction between three kinds of symmetry: which we call `stipulated', `accidental' and `proper'.},
issn={1573-0964},
doi={10.1007/s11229-019-02258-x},
}

@article{NortonNordstrom,
author = {Norton, John D.},
address = {NEW YORK},
copyright = {1993 INIST-CNRS},
issn = {0003-9519},
journal = {Archive for history of exact sciences},
keywords = {Electrons ; Gravitation ; Gravitational fields ; Mass ; Mathematics ; Physical sciences ; Relativity},
language = {eng},
number = {1},
pages = {17-94},
title = {Einstein, Nordström and the Early Demise of Scalar, Lorentz-Covariant Theories of Gravitation},
volume = {45},
year = {1992},
publisher = {Springer-Verlag},
}

@misc{pittphilsci22172,
            year = {2023},
          author = {Patrick D{\"u}rr and James Read},
           title = {{Reconsidering Conventionalism: An Invitation to a Sophisticated Philosophy for Modern (Space-)Times}},
           month = {May},
        keywords = {Conventionalism, underdetermination, spacetime theories},
        note = {Phil. Sci. Archive 22172},
}


@Article{GeometricalTrinity,
AUTHOR = {Beltrán Jiménez, Jose and Heisenberg, Lavinia and Koivisto, Tomi S.},
TITLE = {The Geometrical Trinity of Gravity},
JOURNAL = {Universe},
VOLUME = {5},
YEAR = {2019},
NUMBER = {7},
ARTICLE-NUMBER = {173},
ISSN = {2218-1997},
ABSTRACT = {The geometrical nature of gravity emerges from the universality dictated by the equivalence principle. In the usual formulation of General Relativity, the geometrisation of the gravitational interaction is performed in terms of the spacetime curvature, which is now the standard interpretation of gravity. However, this is not the only possibility. In these notes, we discuss two alternative, though equivalent, formulations of General Relativity in flat spacetimes, in which gravity is fully ascribed either to torsion or to non-metricity, thus putting forward the existence of three seemingly unrelated representations of the same underlying theory. Based on these three alternative formulations of General Relativity, we then discuss some extensions.},
DOI = {10.3390/universe5070173}
}

@misc{NonRelTrinity,
      title={The Non-Relativistic Geometric Trinity of Gravity}, 
      author={William J. Wolf and James Read and Quentin Vigneron},
      year={2024},
      eprint={2308.07100},
      archivePrefix={arXiv},
      primaryClass={gr-qc}, 
}

@article{CoffeyKevin2014TEaI,
author = {Coffey, Kevin},
address = {Oxford},
copyright = {British Society for the Philosophy of Science 2014},
issn = {0007-0882},
journal = {The British journal for the philosophy of science},
keywords = {Judgment ; Philosophy ; Physics ; Quantum theory},
language = {eng},
number = {4},
pages = {821-844},
title = {Theoretical Equivalence as Interpretative Equivalence},
volume = {65},
year = {2014},
publisher = {Oxford University Press},
}


